Piezoelectric polymer generators: the large bending regime

There is an important difference between piezoelectric polymer films and solid crystals for the application to piezoelectric generators. In the case of polymers, the optimal piezoelectric response imposes {\it a large bending regime}. Starting from the linear Curie's constitutive equations, we develop an analytical model under the assumption of the large bending regime resulting from bulge testing configuration. This model shows a specific non-linear piezoelectric response, that follows a power $2/3$ of the mechanical excitation. The piezoelectric voltage and the corresponding power are then studied experimentally as a function of the angular frequency $\omega$ of the mechanical excitation, the load resistance $R$, and the thickness of the film $\ell$. The experimental results carried out on piezoelectric PVDF films validate the model.

==> bib/newbiblio.tex <==
\bibitem{Timoshenko1959THEORYOP}
Stephen P. Timoshenko and S. Woinowsky-Krieger
{\it THEORY OF PLATES AND SHELLS} (1959),
https://api.semanticscholar.org/CorpusID:137571381


\bibitem{Here1973AcousticFA}
Bert A. Auld, {\it Acoustic fields and waves in solids, McGraw-Hill publisher 1973},
https://api.semanticscholar.org/CorpusID:122055062

\bibitem{Mo_2014}
Changki Mo and Joseph Davidson and William W Clark
{\it Energy harvesting with piezoelectric circular membrane under pressure loading}
Smart Materials and Structures {\bf 23}, 045005 (2014),
doi = 10.1088/0964-1726/23/4/045005,

\bibitem{en17163886}
Wang, Xinyue and Zuo, Jialin and Jiang, Tianlin and Xiao, Jinxin and Tong, Jie and Huang, Shiqing and Zhang, Wenhua,
{\it Analysis of Vibration Electromechanical Response Behavior of Poly(Vinylidene Fluoride) Piezoelectric Films},
Energies {\bf 17}, 3886 (2024),
DOI = 10.3390/en17163886

\bibitem{Dedkova2020}
Dedkova, Anna A. and Yu. Glagolev, Petr and Demin, Gleb D. and Gusev, Evgeney E. and Skvortsov, Pavel A.,
{\it Mechanical Stresses Analysis of Thin Round Membranes in the Case of Large Deflections}
2020 IEEE Conference of Russian Young Researchers in Electrical and Electronic Engineering (EIConRus), 
(2020), 10.1109/EIConRus49466.2020.9039289

\bibitem{nano13061098}
Sasmal, Abhishek and Senthilnathan, Jaganathan and Arockiarajan, Arunachalakasi and Yoshimura, Masahiro,
{\it Two-Dimensional Metal-Organic Framework Incorporated Highly Polar PVDF for Dielectric Energy Storage and Mechanical Energy Harvesting},
Nanomaterials {\bf 13}, 1098 (2023),
DOI = 10.3390/nano13061098,

\bibitem{NAVAL2023114330}
Sourav, Naval and Pratibha, Verma and Ankesh, Jain and Dhiman, Mallick
{\it Hybrid vector and pressure sensor for fingertip dynamics sensing using DC-triboelectric/AC-piezoelectric mechanisms},
Sensors and Actuators A: Physical {\bf 355}, 114330 (2023),
doi = https://doi.org/10.1016/j.sna.2023.114330,


\bibitem{WANG2023}
Sasa, Wang and Asif Abdullah, Khan and Sam, Teale and Jian, Xu and Darshan, H. Parmar and Ruyan, Zhao and Luke, Grater and Peter, Serles and Yu, Zou and Tobin, Filleter and Dwight, S. Seferos and Dayan, Ban and Edward, H. Sargent
{\it Large piezoelectric response in a Jahn-Teller distorted molecular metal halide},
Nature Communications {\bf 14}, 1852 (2023),
doi = https://doi.org/10.1038/s41467-023-37471-3,

\bibitem{HASSANPOURAMIRI2023}
Morteza {Hassanpour Amiri} and Rose Fatscher and Rebecca Taylor and Paulo R.F. Rocha and Chris R. Bowen and Kamal Asadi, 
{\it Piezoelectric energy harvesters: A critical assessment and a standardized reporting of power-producing vibrational harvesters},
Nano Energy {\bf 106}, 108073 (2023),
doi = https://doi.org/10.1016/j.nanoen.2022.108073


\bibitem{Figure_merit}
Deutz, Daniella B. and Pascoe, John-Alan and Schelen, Ben and van der Zwaag, Sybrand and de Leeuw, Dago M. and Groen, Pim",
{\it Analysis and experimental validation of the figure of merit for piezoelectric energy harvesters},
Mater. Horiz. {\bf 5}, 444-453 (2018)
doi  ="10.1039/C8MH00097B",

\bibitem{Peigney_2013}
Michael Peigney and Dominique Siegert
{\it Piezoelectric energy harvesting from traffic-induced bridge vibrations},
Smart Materials and Structures {\bf 22}, 095019 (2013)
doi = {10.1088/0964-1726/22/9/095019},

\bibitem{reviewpipeline202300235}
Li, Zihe and Roscow, James and Khanbareh, Hamideh and Haswell, Geoff and Bowen, Chris
{\it Energy Harvesting from Water Flow by Using Piezoelectric Materials},
Advanced Energy and Sustainability Research {\bf 5}, 2300235 (2024)
doi = {https://doi.org/10.1002/aesr.202300235},

\bibitem{Granstrom2007}
Jonathan Granstrom and Joel Feenstra and Henry A Sodano and Kevin Farinholt
{\it Energy harvesting from a backpack instrumented with piezoelectric shoulder straps}
Smart Materials and Structures {\bf 16}, 1810 (2007)
doi = 10.1088/0964-1726/16/5/036,

\bibitem{Nilsson2013}
Erik Nilsson and Anja Lund and Christian Jonasson and Christer Johansson and Bengt Hagstr\"om
{\it Poling and characterization of piezoelectric polymer fibers for use in textile sensors},
Sensors and Actuators A {\bf 201}, 477 (2013),
doi = https://doi.org/10.1016/j.sna.2013.08.011,

\bibitem{Zhang2013}
Zhang, Lei and Oh, Sharon Roslyn and Wong, Ting Chong and Tan, Chin Yaw and Yao, Kui,
{\it Piezoelectric polymer multilayer on flexible substrate for energy harvesting}
IEEE Transactions on Ultrasonics, Ferroelectrics, and Frequency Control {\bf 60}, 2013-2020 (2013),
  doi=10.1109/TUFFC.2013.2786

\bibitem{IEEE_standard}
 IEEE Transactions on Ultrasonics, Ferroelectrics, and Frequency Control, 
{\it Publication and Proposed Revision of ANSI/IEEE Standard 176-1987 "ANSI/IEEE Standard on Piezoelectricity"} 
  {\bf 43}, 717 (1996)
  doi= 10.1109/TUFFC.1996.535477


\bibitem{Uchino}
Uchino, Kenji,
{\it Piezoelectric Energy Harvesting Systems - Essentials to Successful Developments},
Energy Technology {\bf 6}, 829-848 (2018)
doi = https://doi.org/10.1002/ente.201700785,

\bibitem{Jeong}
Jeong, Chang Kyu and Baek, Changyeon and Kingon, Angus I. and Park, Kwi-Il and Kim, Seung-Hyun,
{\it Lead-Free Perovskite Nanowire-Employed Piezopolymer for Highly Efficient Flexible Nanocomposite Energy Harvester},
Small {\bf 14}, 1704022 (2018)
doi = https://doi.org/10.1002/smll.201704022,

\bibitem{POTRZEBOWSKA2021102528}
Natalia Potrzebowska and Olivier Cavani and Ozlem Oral and Olivier Doar\'e and Giuseppe Melilli and Jean-Eric Wegrowe and Marie-Claude. Clochard
{\it Mixing nanostructured Ni/piezoPVDF composite thin films with e-beam irradiation: A beneficial synergy to piezoelectric response},
Materials Today Communications {\bf 28}, 102528 (2021),
doi = https://doi.org/10.1016/j.mtcomm.2021.102528,



